A Radio Flare in the Long-Lived Afterglow of the Distant Short GRB 210726A: Energy Injection or a Reverse Shock from Shell Collisions?

We present the discovery of the radio afterglow of the short $\gamma$-ray burst (GRB) 210726A, localized to a galaxy at a photometric redshift of $z\sim 2.4$. While radio observations commenced $\lesssim 1~$day after the burst, no radio emission was detected until $\sim11~$days. The radio afterglow subsequently brightened by a factor of $\sim 3$ in the span of a week, followed by a rapid decay (a "radio flare"). We find that a forward shock afterglow model cannot self-consistently describe the multi-wavelength X-ray and radio data, and underpredicts the flux of the radio flare by a factor of $\approx 5$. We find that the addition of substantial energy injection, which increases the isotropic kinetic energy of the burst by a factor of $\approx 4$, or a reverse shock from a shell collision are viable solutions to match the broad-band behavior. At $z\sim 2.4$, GRB 210726A is among the highest redshift short GRBs discovered to date as well as the most luminous in radio and X-rays. Combining and comparing all previous radio afterglow observations of short GRBs, we find that the majority of published radio searches conclude by $\lesssim 10~$days after the burst, potentially missing these late rising, luminous radio afterglows.

==> RefereeResponse.tex <==
In my view, the manuscript "A Radio Flare in the Long-Lived Afterglow of the Distant Short GRB 210726A:.." presents a thorough analysis of a short GRB with several remarkable aspects that render it of sufficient interest for a dedicated paper on the event. The manuscript is well-written with a clear narrative progression. I therefore would be happy to recommend this work for publication once the points below are taken into account. This would be a request for moderate revision at most, certainly not major, with point 2 probably the most substantial.

1. Other than the unexpected radio flaring behavior, the burst is an outlier in terms of its distance which is relatively large for a short GRB. This distance is however determined not from spectral lines but from a modeling of the host galaxy using a stellar population modeling code called Prospector. It is not clear to me how original this approach is. Can the authors provide a bit more context here? If there is a precedent in determining GRB redshifts in this or similar manner, some relevant citations would be useful. If this is a novel approach, then the authors are well within their rights to emphasize this as such more than they currently do.

%We thank the referee for their comment. We have added a footnote to section 3.2 to explain that the use of Prospector to determine photometric redshifts is common within the short GRB community (i.e. O'Connor et al. 2022, 2022MNRAS.515.4890O; Nugent et al. 2022 2022ApJ...940...57N). We use Propspector as it is a powerful galaxy modeling code given its Bayesian inference model that produces realistic uncertainties on host galaxy properties (Leja et al. 2017 2017ApJ...837..170L). Additionally, Prospector has been generally adopted within the transient community for determining host galaxy properties, i.e. CCSNe (Schulze et al. 2021, 2021ApJS..255...29S), FRBs (Gordon et al. 2023, 2023ApJ...954...80G), Type Ia SNe (Nugent et al. 2023 2023arXiv230410601N), Ca-rich Transients (Dong et al. 2022 2022ApJ...927..199D). 

2. A consequence of the method that is used to determine the redshift is that z is only known within a broad range. The value of z will impact different spectral regimes differently, and the corresponding luminosity distance will impact the overall flux levels across the board (the difference between z = 2.4 as inferred for this burst and median sample z = 0.64 being about a factor 5 in luminosity distance). I therefore expect the outcome of the fit, including the relative match to various regimes, to be sensitive to z, when z is allowed to vary over the range indicated in Figure 4 of the manuscript. Further, z = 2.4 is a clear outlier for short GRBs. I therefore think that the authors should examine the impact of z more systematically than they currently do. Leaving z as a fit parameter in afterglow analysis is typically not meaningful, given the lack of features of synchtron spectra, but in this case, the authors will have the benefit of a well-defined prior when including z in the fit: the posterior as shown in Fig 4, or any reasonably (semi-)analytic approximation of that shape. Including this posterior from Prospector as prior in the afterglow modelling should be straightforward thanks to the versatility on this front of the emcee code used by the authors, and doing so would effectively amount to a joint fit of the galaxy and the afterglow, an interesting novelty on its own. It would also render the results, and any arguments for additional components, more robust in general.

% We thank the referee for this insightful comment and suggestion for how to improve our afterglow fits. Upon receiving this comment, we were motivated to implement a new module in our afterglow fitting code to intake a redshift prior, as mentioned in section 5.2. Given that the large majority of the Prospector posterior probability resides at z>2, we found that this implementation did not significantly change the afterglow properties. The highest likelihood redshift was z=2.74, and the median was z=2.29+0.44-0.63. As a result, no parameter changed outside of the 1 sigma values. We therefore present the derived property values in Table 4 but proceed with the discussion using our fixed redshift properties.

3. A last point related to redshift. Given that observer time is related to burster time by a factor (1+z), I think that the timescales of any features in the afterglow inherit this proportionality. Comparing again z = 2.4 and z = 0.64, this amounts to a factor of two that I would like to see reflected in the discussion. For example, should we be considering delta t > ~5 days rather than 10 days, in the discussion about for how long and when to follow-up short GBRs in the radio (section 7.3)?

% We thank the referee for pointing out this important caveat. We have included a clarification in 7.1.3 that if the X-ray rebrightening observed at 4.6 days is indicative of central engine activity, this relates to a rest-frame time of 1.4 days.  We also included a footnote in 7.3 to address the rest frame time, explaining that delta t ~ 10 days is merely a general benchmark, as the the redshift, and therefore the rest frame time, of a short GRB is not typically known until well after radio observations have concluded. We also noticed a mistake on our part, in section 7.2 we reference X-ray luminosity at a common rest frame time, but did not state as such. We have adjusted our text accordingly. 

4. In 5.2 it is mentioned that the high value for epsilon_E can be brought down by bringing down f_NT. But if this is subject to the degeneracy outlined by Eichler & Waxman, that this would also bring down epsilon_B (already low), and raise E and N_0. Can the authors comment on this?

% We have included several sentences commenting on the effect of f_NT < 1 within Appendix B. We find that the change in epsilon_B is not concerning, as several studies of GRB afterglows have found low values of epsilon_B of 1e-5. Furthermore, given our derived n_0 is within the typical short GRB population, an order of magnitude increase would not be concerning. However, given the high E derived by our fits, due to the high redshift, any increase would provide further proof that GRB 210726A is superlative in it's afterglow properties.

further minor points:
% We appreciate the referee's attention to detail and have adjusted the text to address the minor points accordingly.

- typo in section 2.1.2, "The source was was"


- On page 13, bottom left, "The resulting value" for the jet opening angle is mentioned directly following a statement about optical extinction within the same paragraph. Presumably we should not infer that optical non-detections require a wide opening angle?

- The manuscript is careful to identify triangles as indicating upper limits in all relevant figure captions except for that of Fig 5. Maybe point this out here too?


% In addition to the changes requested by the referee, we also simplified our discussion of the reverse shock model. Upon discussion with co-authors and a community scientist attempting to use the equations we previously had section 6.2, we realized that our model to explain this GRB does not hinge upon the equations, which outlined a relation between the RS and FS. Furthermore, these relations have not broadly been tested on other GRBs that invoke a two shell model, and upon further thought we are not convinced they were physically sound - so we have removed them. We emphasize that our results do not change, and we can still have viable RS model without these assumptions.

% We have also removed some of our discussion about Klein Nishina effects (Section 5.2, 2nd paragragh), as the details are discussed more thoroughly in a separate paper and KN corrections are not the focus of this work.
